No-Regret Learning in Partially-Informed Auctions

Auctions with partially-revealed information about items are broadly employed in real-world applications, but the underlying mechanisms have limited theoretical support. In this work, we study a machine learning formulation of these types of mechanisms, presenting algorithms that are no-regret from the buyer's perspective. Specifically, a buyer who wishes to maximize his utility interacts repeatedly with a platform over a series of $T$ rounds. In each round, a new item is drawn from an unknown distribution and the platform publishes a price together with incomplete, "masked" information about the item. The buyer then decides whether to purchase the item. We formalize this problem as an online learning task where the goal is to have low regret with respect to a myopic oracle that has perfect knowledge of the distribution over items and the seller's masking function. When the distribution over items is known to the buyer and the mask is a SimHash function mapping $\mathbb{R}^d$ to $\{0,1\}^{\ell}$, our algorithm has regret $\tilde O((Td\ell)^{1/2})$. In a fully agnostic setting when the mask is an arbitrary function mapping to a set of size $n$ and the prices are stochastic, our algorithm has regret $\tilde O((Tn)^{1/2})$.

==> sec/finite_sample_ETC.tex <==
\section{General Strategy with Adversarial Prices}\label{sec:finite-sample}

In practice, the prices may often be non-stochastic and can be generated strategically by the seller to maximize revenue. In this section, we consider a more challenging setting with an unknown item distribution and adversarial prices. At each time step $t\in [T]$, $\vx_t$ is drawn from an unknown item distribution $\cP$. The published prices $p_t(\vx_t)$ are now assumed to be generated by an oblivious adversary. To be robust to such an adversary, the algorithm we present uses a classic ``explore-then-commit'' approach. We prove that
it achieves $\tilde \cO(T^{\nicefrac{3}{4}}n^{\nicefrac{1}{2}})$ regret even in this challenging setting. We present the details in Algorithm~\ref{alg:unknown-prob}. %For each $i \in [n]$, we use the notation $\eta_i = \Pr_{\vx \sim \cP}[h(\vx) = i]$ and $v_i = \E[v^*(\vx) \mid h(\vx) = i]$. 


% We now study the \emph{finite sample model}, where the distribution $\cP$ over items is unknown. In this setting, our model is more general than that of Section~\ref{sec:population}, but our regret bound grows with $T^{\nicefrac{3}{4}}$ rather than $T^{\nicefrac{1}{2}}$. In particular,
% the item $\vx$ is an element of some abstract set $\cX$ (for example, $\cX$ might equal $\R^d$ as in Section~\ref{sec:population}, but it could also equal any other set). There are $n$ sets $S_1, \dots, S_n$ partitioning $\cX$. At each time step $t\in [T]$, $\vx_t$ is drawn from  $\cP$. Then the set index $h(\vx_t) \in [n]$ such that $\vx_t \in S_{h(\vx_t)}$ is revealed. For each $i \in [n]$, let $\eta_i = \Pr[\vx \in S_i]$ and $v_i = \E[v^*(\vx) \mid \vx \in S_i]$.


% Then the set index $h(\vx_t) \in [n]$ such that $\vx_t \in S_{h(\vx_t)}$ is revealed. For each $i \in [n]$, let $\eta_i = \Pr[\vx \in S_i]$ and $v_i = \E[v^*(\vx) \mid \vx \in S_i]$.

\subsection{Explore-then-commit with unknown $\cP$}

\begin{algorithm}[!ht]
\caption{Explore-then-Commit (Unknown Distribution)}\label{alg:unknown-prob}
\begin{algorithmic}[1]
\STATE \textbf{Input: horizon $T$, exploration phase length $t' \geq 1$.}
\STATE For each $i \in [n]$, set $\hat{\eta}_i \leftarrow 0$ and $\hat{v}_i \leftarrow 0$.
\FOR[\textcolor{blue}{Exploration phase}]{$t=1,2,\ldots, t'$}
\STATE Receive $h(\vx_t)$, price $p_t(\vx_t)$ where $\vx_t \stackrel{iid}{\sim} \cP$.
\STATE Make decision $b_t = 1$ and observe $v^*(\vx_t)$.
\STATE Set $\hat{\eta}_{h(\vx_t)} \leftarrow \hat{\eta}_{h(\vx_t)} + \frac{1}{t'}.$
\STATE Set $\hat{v}_{h(\vx_t)} \leftarrow \hat{v}_{h(\vx_t)} + \frac{v^*(\vx_t)}{t'}.$
\ENDFOR\\[1ex]

\FOR[\textcolor{blue}{Exploitation phase}]{$t=t'+1, t' + 2, \ldots, T$}
\STATE Receive $h(\vx_t)$, price $p_t(\vx_t)$ where $\vx_t \stackrel{iid}{\sim} \cP$.
\STATE Compute estimate \[\hat Z_t \defeq \begin{cases} \frac{\hat{v}_{h(\vx_t)}}{\hat{\eta}_{h(\vx_t)}} &\text{if } \hat{\eta}_{h(\vx_t)} > 0\\
0 &\text{otherwise.}\end{cases}\]
\STATE Make decision $b_t = \Ind(\hat Z_t \geq p_t(\vx_t))$.
\ENDFOR\\[1ex]
\end{algorithmic}
\end{algorithm}

%There are $n$ sets $S_1, \dots, S_n$ partitioning $\cX$. At each time step $t\in [T]$, $\vx_t$ is drawn from  $\cP$. Then the set index $h(\vx_t) \in [n]$ such that $\vx_t \in S_{h(\vx_t)}$ is revealed. For each $i \in [n]$, let $\eta_i = \Pr[\vx \in S_i]$ and $v_i = \E[v^*(\vx) \mid \vx \in S_i]$. 

Algorithm~\ref{alg:unknown-prob} begins with an exploration phase of length $t'$. For every round $t \in [t']$ the buyer always buys the item. During the exploration, the algorithm maintains an estimate $\hat{\eta}_i$ of $\eta_i:=\Pr_{\vx \sim \cP}[h(\vx) = i]$ and $\hat{v}_i$ of $v_i:=\E[v^*(\vx) \Ind(h(\vx) = i)]$. In Lemma~\ref{lem:estimate_conditional}, we show that if $\eta_i$ is sufficiently large, then $\hat{v}_i/\hat{\eta}_i$ approximates $\E[v^*(\vx) \mid h(\vx) = i]$---which is the key threshold for the optimal policy (see Prop.~\ref{prop:opt}). The remainder of the rounds $t\in \{t' + 1, t'+2, \dots, T\}$ are exploitation rounds: the buyer buys the item if and only if $\hat{v}_{h(\vx_t)}/\hat{\eta}_{h(\vx_t)} \geq p_t(\vx_t)$.

\subsection{Regret analysis}

We begin our analysis by proving that with high probability, for any $i \in [n]$ such that $\eta_i$ is sufficiently large, $\hat{v}_i/\hat{\eta}_i$ approximates $\E[v^*(\vx) \mid h(\vx) = i]$.

\begin{restatable}{lemma}{estimateConditional}\label{lem:estimate_conditional}
For any $\beta \geq \frac{9}{t'} \ln \frac{4n}{\delta}$, with probability $1 - \delta$, for every $i \in [n]$ such that $\eta_i \geq \beta$, at the end of the exploration phase, $\hat{\eta}_i > 0$ and \[\left|\E\left[v^*(\vx)\mid h(\vx) = i\right] - \frac{\hat{v}_i}{\hat{\eta}_i}\right| \leq 25H\sqrt{\frac{1}{\beta t'}\ln \frac{4n}{\delta}}.\]
\end{restatable}

\begin{proof}[Proof sketch]
Our proof begins with the observation that for any index $i \in [n]$, we have
\[\E\left[v^*(\vx) \mid h(\vx) = i\right] = \frac{\E[v^*(\vx) \Ind(h(\vx) = i)]}{\Pr[h(\vx) = i]} = \frac{v_i}{\eta_i}.\] 
We then use this fact to bound the difference between $\E\left[v^*(\vx) \mid h(\vx) = i\right]$ and $\frac{\hat{v}_i}{\hat{\eta}_i}$.

Beginning with the numerator, recall that $\hat{v}_i$ is an empirical estimate of $v_i$. By Bernstein's inequality~\citep[see, e.g.,][]{Haussler92:Decision}, with probability at least $1 - \frac{\delta}{2n}$, we have that \[\frac{(1 - \alpha)v_i - H\alpha\beta}{1 + \alpha} \leq \hat{v}_i \leq \frac{(1 + \alpha)v_i + H\alpha\beta}{1 - \alpha},\] where $\alpha =  \sqrt{\frac{1}{\beta t'} \ln \frac{4n}{\delta}}$. Moving to the denominator, by a Chernoff-Hoeffding bound~\citep{boucheron2013concentration}, we know that with probability at least $1 - \frac{\delta}{2n}$, \[\left(1 - 2\alpha\right)\eta_i \leq \hat{\eta}_i \leq \left(1 + 2\alpha\right)\eta_i.\] 
% By definition of $\beta$, we know that $\alpha \leq \frac{1}{3}$, so $\hat{\eta}_i > 0$. 

The rest of the proof combines these two high-probability bounds. We provide the full proof in Appendix~\ref{app:finite-sample}.
\end{proof}
% we have that with high probability:
% \begin{align*}\frac{\hat{v}_i}{\hat{\eta}_i} &\leq \frac{v_i}{\eta_i}\cdot \frac{1 + \alpha}{(1-\alpha)(1 - 2\alpha)} + \frac{H\alpha \beta}{\eta_i(1-\alpha)(1-2\alpha)}\\
% &\leq \frac{v_i}{\eta_i}\cdot \frac{1 + \alpha}{(1-\alpha)(1 - 2\alpha)} + \frac{H\alpha }{(1-\alpha)(1-2\alpha)},\end{align*} where the second inequality follows from the fact that $\beta \leq \eta_i$. Rearranging terms, we have that \begin{align}\frac{\hat{v}_i}{\hat{\eta}_i} &\leq \frac{v_i}{\eta_i}\cdot \left(1 + \frac{4\alpha - 2\alpha^2}{(1-\alpha)(1-2\alpha)}\right) + \frac{H\alpha}{(1-\alpha)(1-2\alpha)}\nonumber\\
% &\leq \frac{v_i}{\eta_i}\cdot \left(1 + \frac{4\alpha}{(1-\alpha)(1-2\alpha)}\right) + \frac{H\alpha}{(1-\alpha)(1-2\alpha)}\nonumber\\
% &\leq \frac{v_i}{\eta_i}\cdot \left(1 + 20\alpha\right) + 5H\alpha,\label{eq:rearrange}\end{align} where the final inequality follows from the fact that $\alpha \leq \frac{1}{3}$. Next, we use the fact that \begin{align*}\frac{v_i}{\eta_i} &= \frac{\E[v^*(\vx) \Ind(\vx \in S_i)]}{\Pr[\vec{x} \in S_i]} \leq \frac{\E[H \cdot \Ind(\vx \in S_i)]}{\Pr[\vec{x} \in S_i]}\\
% &= \frac{H\Pr[\vec{x} \in S_i]}{\Pr[\vec{x} \in S_i]} = H.\end{align*} This inequality and Equation~\eqref{eq:rearrange} imply that \[\frac{\hat{v}_i}{\hat{\eta}_i} \leq \frac{v_i}{\eta_i} + 25H\alpha  = \frac{v_i}{\eta_i} + 25H\sqrt{\frac{1}{\beta t'}\ln \frac{4n}{\delta}}.\]

% The proof that \[\frac{\hat{v}_i}{\hat{\eta}_i} \geq \frac{v_i}{\eta_i} + 25H\sqrt{\frac{1}{\beta t'}\ln \frac{4n}{\delta}}\] follows by a symmetric argument and can be found 

We now prove a bound on the instantaneous expected regret of Algorithm~\ref{alg:unknown-prob} during the exploitation rounds assuming that the high-probability event from Lemma~\ref{lem:estimate_conditional} holds. 
The proof is similar to that of Lemma~\ref{lem:loss-diff} and can be found in Appendix~\ref{app:finite-sample}.

\begin{restatable}{lemma}{goodEvent}\label{lem:good_event}
Suppose that for every $i \in [n]$ such that $\eta_i \geq \beta$, at the end of the exploration phase, $\hat{\eta}_i > 0$ and \[\left|\E\left[v^*(\vx)\mid h(\vx) = i\right] - \frac{\hat{v}_i}{\hat{\eta}_i}\right| \leq 25H\sqrt{\frac{1}{\beta t'}\ln \frac{4n}{\delta}}.\]
Then in each round of the exploitation phase in Algorithm~\ref{alg:unknown-prob}, the expected regret incurred in that round is \[H\left(25\sqrt{\frac{1}{\beta t'}\ln \frac{4n}{\delta}} + \beta n\right).\]
\end{restatable}

We next use Lemma~\ref{lem:good_event} to bound the regret of Algorithm~\ref{alg:unknown-prob}.

\begin{restatable}{lemma}{anyBeta}\label{lem:any_beta} For any $\beta \geq \frac{9\ln (4nT)}{t'}$, Algorithm~\ref{alg:unknown-prob} has an expected regret of
\begin{equation}\E[R_T] \leq H\left(t' + 1 + \beta n T + 25T \sqrt{\frac{\ln (4nT)}{\beta t'}}\right).\label{eq:beta_regret}
\end{equation}
\end{restatable}

\begin{proof}
First, in the exploration phase, the total regret is upper bounded by $Ht'.$ By the end of the exploration phase, by Lemma~\ref{lem:estimate_conditional}, we know that with probability $1 - \frac{1}{T}$, for every $i \in [n]$ such that $\eta_i > \beta$, we have seen at least one sample with $h(\vx) = i$ (i.e., $\hat{\eta}_i > 0$) and we can estimate the conditional expected value \begin{equation}\left|\E\left[v^*(\vx)\mid h(\vx) =i\right] - \frac{\hat{v}_i}{\hat{\eta}_i}\right| \leq 25H\sqrt{\frac{\ln (4nT)}{\beta t'}}.\label{eq:inst_reg}\end{equation} In other words, the conditions from Lemma~\ref{lem:good_event} hold. With probability $\frac{1}{T}$, these two conditions fail to hold, in which case the instantaneous utility loss at each round may be as high as $H$, which contributes $H \cdot \frac{1}{T} \cdot T = H$ to the total expected regret. Otherwise, suppose that the conditions from Lemma~\ref{lem:good_event} hold. By Lemma~\ref{lem:good_event}, the instantaneous utility loss is at most $H\left(25\sqrt{\frac{\ln (4nT)}{\beta t'}} + \beta n\right)$, which contributes $HT\left(25\sqrt{\frac{\ln (4nT)}{\beta t'}} + \beta n\right)$ to the total expected regret. Therefore, the theorem statement holds.
\end{proof}


In Theorem~\ref{thm:finite_regret}, we set $\beta$ and $t'$ to be sublinear in $T$, which implies that Algorithm~\ref{alg:unknown-prob} is no-regret.

\begin{restatable}{theorem}{finiteRegret}\label{thm:finite_regret}
Algorithm~\ref{alg:unknown-prob} with $t' = T^{\nicefrac{3}{4}}n^{\nicefrac{1}{2}}\ln (4nT)$ has an expected regret of $\E[R_T] = O(HT^{\nicefrac{3}{4}}n^{\nicefrac{1}{2}}\ln (nT)).$
\end{restatable}

\begin{proof}
This follows from Lemma~\ref{lem:any_beta} by setting $\beta = 9T^{-\nicefrac{1}{4}}n^{-\nicefrac{1}{2}}$ which satisfies $\beta \geq \frac{9\ln (4nT)}{t'}$.
\end{proof}

In the following theorem, we prove that if we know the minimum probability $\tilde{\eta} \defeq \min \{\eta_i : \eta_i > 0\}$, then we can improve the dependence on $T$ in the regret bound from $T^{\nicefrac{3}{4}}$ to $T^{\nicefrac{2}{3}}$.

\begin{restatable}{theorem}{finiteRegret2}\label{thm:finite_regret_known_t}
Suppose that $\tilde{\eta}$ is known. Then Algorithm~\ref{alg:unknown-prob}, with $t' = 9T^{\nicefrac{2}{3}}\tilde{\eta}^{-1}\ln (4nT)$, has an expected regret of $\E[R_T] = O(HT^{\nicefrac{2}{3}}\tilde{\eta}^{-1}\ln (nT)).$
\end{restatable}

\begin{proof}
This proof follows by the same logic as the proof of Lemma~\ref{lem:any_beta} with $\beta = \tilde{\eta}$, which satisfies the inequality $\beta \geq \frac{9\ln (4nT)}{t'}$. However, we can remove the term $H\beta n T$ from the bound on $\E[R_T]$ from Equation~\eqref{eq:beta_regret} since by definition of $\tilde{\eta}$, there are no rounds $t \in [T]$ where $h(\vx_t) =i$ with $\eta_i < \beta = \tilde{\eta}$. Therefore, we have that $\E[R_T] \leq H\left(t' + 1 + 50T \sqrt{\frac{\ln (4nT)}{\tilde{\eta} t'}}\right) = O(HT^{\nicefrac{2}{3}}\tilde{\eta}^{-1}\ln (nT)).$
\end{proof}

\begin{remark}
We make some further comments in the sequel. First, note that similar to Algorithm~\ref{alg:explore-then-commit}, Algorithm~\ref{alg:exp4} and Algorithm~\ref{alg:unknown-prob} assumed that the horizon $T$ was known. Again this assumption can be lifted via a doubling trick. Second, apart from Algorithm~\ref{alg:unknown-prob}, under the same setting, one can also consider applying one copy of a known bandit algorithm (such as Algorithm~\ref{alg:unknown-prob} with $n=1$, or Algorithm (Eq. 8.3) in~\citet{slivkins2019introduction}) to items that belong to each bucket. In other words, one can run $n$ copies of that algorithm in parallel, where each algorithm handles the items that belong to one single bucket. By doing so, the dependence on $n$ can be improved. Running $n$ copies of Algorithm~\ref{alg:unknown-prob} with $n=1$ leads to a regret bound $\tilde O(T^{3/4}n^{1/4})$. However, we will need to apply the doubling trick to each individual algorithm even when $T$ is given, because the horizon for each algorithm is unknown.
\end{remark}

% in general if each copy has regret T^alpha, total regret is T^\alpha n^{1-alpha}












% \textcolor{red}{EARLIER NOTES:}

% \begin{itemize}
%     \item The learned vectors $\hat{\vec{w}}_1, \dots, \hat{\vec{w}}_p$ partition $\R^d$ into $k \leq 2^p$ regions $S_1, \dots, S_k$.
%     \item Given a set of samples $\vec{x}_1, \dots, \vec{x}_N$, we want to be able to estimate \[\E[v^*(\vec{x}) \mid \vec{x} \in S_i] = \frac{\E[v^*(\vec{x}) \Ind(\vec{x} \in S_i)]}{\Pr[\vec{x} \in S_i]}\] for any $i \in [k]$.
%     \item For any $i \in [k]$ and let $\Pr[\vec{x} \in S_i] = p_i$ and let $\hat{p}_i = \frac{1}{N} \sum_{j = 1}^N\Ind(\vec{x}_j \in S_i)$. From a Chernoff bound, \[\Pr\left[p_i(1-\gamma) \leq \hat p_i \leq p_i(1+\gamma)\right] \geq 1 - 2\exp\left(\frac{-\gamma^2p_iN}{2}\right).\] In other words, given $N = O\left(\frac{2}{\gamma^2p_i}\ln \frac{2}{\delta}\right)$ samples, this bound holds with probability $1-\delta.$
    
%     \wg{(by Chernoff-Hoeffding):}
%     \[\Pr\left[p_i(1-\gamma) \leq \hat p_i \leq p_i(1+\gamma)\right] \geq 1 - 2\exp\left(-\frac{\gamma^2}{2+\gamma}Np_i\right).\]
%     \begin{itemize}
%       \item How to deal with the fact that $p_i$ shows up in this sample complexity bound?
%         \begin{itemize}
%             \item Intuitively, even if a dependence on $p_i$ is necessary, the privacy-preserving aspect of the problem would intuitively mean that if $p_i \not=0$, then $p_i$ shouldn't be too small...
%         \end{itemize}
%     \end{itemize}
%     \item To estimate $\E[v^*(\vec{x}) \Ind(\vec{x} \in S_i)]$, let $v_i = \E[v^*(\vec{x}) \Ind(\vec{x} \in S_i)]$ and $\hat{v}_i = \frac{1}{N} \sum_{j = 1}^N v^*(\vec{x}_j) \Ind(\vec{x}_j \in S_i)$. Then with probability $1-\delta$ over the draw of $N = \tilde{O}\left(\frac{1}{\alpha^2\nu}\right)$ samples, \[\frac{|v_i - \hat{v}_i|}{v_i + \hat{v}_i + H\nu} \leq \alpha.\] Written another way, \[\frac{(1-\alpha)v_i - H\alpha\nu}{1 + \alpha} \leq \hat{v}_i \leq \frac{(1 + \alpha)v_i + H\alpha \nu}{1 - \alpha}.\] This follows from a result by \citet{li2001improved}. Here $\nu$ is an adjustable parameter.
%     \item Recall that we have 
% \[
% (1-\gamma)p_i\leq \hat p_i \leq (1+\gamma)p_i,
% \]
% and
% \[\frac{(1-\alpha)v_i - H\alpha\nu}{1 + \alpha} \leq \hat{v}_i \leq \frac{(1 + \alpha)v_i + H\alpha \nu}{1 - \alpha}.\]  We now bound the difference between $\frac{\hat{v}_i}{\hat{p}_i}$ and $\frac{v_i}{p_i}$, setting $\nu = p_i:$
%     \begin{align*}
%         \frac{\hat{v}_i}{\hat{p}_i} &\leq \frac{v_i}{p_i}\cdot \frac{1 + \alpha}{(1-\alpha)(1 - \gamma)} + \frac{H\alpha p_i}{p_i(1-\alpha)(1-\gamma)}\\
%         &= \frac{v_i}{p_i}\cdot \frac{1 + \alpha}{(1-\alpha)(1 - \gamma)} + \frac{H\alpha}{(1-\alpha)(1-\gamma)}\\
%         &= \frac{v_i}{p_i}\cdot \left(1 + \frac{1 + \alpha - (1-\alpha)(1 - \gamma)}{(1-\alpha)(1 - \gamma)}\right) + \frac{H\alpha}{(1-\alpha)(1-\gamma)}\\
%         &= \frac{v_i}{p_i}\cdot \left(1 + \frac{2\alpha + \gamma - \alpha\gamma}{(1-\alpha)(1 - \gamma)}\right) + \frac{H\alpha}{(1-\alpha)(1-\gamma)}\\
%         &\leq \frac{v_i}{p_i}\cdot \left(1 + \frac{2\alpha + \gamma}{(1-\alpha)(1 - \gamma)}\right) + \frac{H\alpha}{(1-\alpha)(1-\gamma)}\\
%         &\leq \frac{v_i}{p_i} + \frac{H(3\alpha + \gamma)}{(1-\alpha)(1-\gamma)} & \left(\frac{v_i}{p_i} \leq H\right)\\
%         &\leq \frac{v_i}{p_i} + 4H(3\alpha + \gamma) & \left(\text{Assuming }\alpha,\gamma \leq \frac{1}{2}\right)\\
%     \end{align*} 
%     {\color{blue}(To be completed: the opposite direction.)}
    
%     If we set $\alpha = \gamma = \frac{\epsilon}{16H}$ then we get an error bound of $\epsilon.$ This requires a sample complexity of $\tilde{O}\left(\frac{H^2}{\epsilon^2p_i}\right).$
% \end{itemize}

% \paragraph{Bounding $\frac{\hat v_i}{\hat p_i}$:}

% By the above,
% \begin{align*}
%     \frac{\hat v_i}{ \hat p_i} &\leq \frac{(1+\alpha)v_i + H\alpha\nu}{1 - \alpha} \frac{1}{(1-\gamma)p_i} \\
%     &\leq \frac{v_i}{p_i} \left(\frac{(1+\alpha)}{(1-\alpha)(1-\gamma)}\right) + \frac{H\alpha \nu }{p_i(1-\alpha)(1-\gamma)}\\
%     &\leq \frac{v_i}{p_i}\left( 1+ \frac{\gamma + \alpha(2+\gamma)}{1-\alpha}\right) + \frac{H\alpha(1+\gamma)}{1-\alpha} \quad (\text{set } \nu = p_i).
% \end{align*}

% The opposite direction:
% \begin{align*}
% \frac{\hat v_i}{ \hat p_i} &\geq \frac{(1-\alpha)v_i - H\alpha\nu}{1 + \alpha} \frac{1}{p_i(1+\gamma)} \\
%     &\geq \frac{v_i}{p_i} \frac{1-\alpha}{(1+\alpha)(1+\gamma)}- \frac{H\alpha \nu }{p_i(1+\alpha)(1+\gamma)}\\
%     &\geq \frac{v_i}{p_i} \left(  1 - \frac{\gamma + 2\alpha+\alpha\gamma}{(1+\alpha)(1+\gamma)}\right) - \frac{H \alpha }{(1+\alpha)(1+\gamma)} \quad (\text{set } \nu = p_i)\\
%     &\geq \frac{v_i}{p_i} - H  \frac{\gamma + 3\alpha+\alpha\gamma}{(1+\alpha)(1+\gamma)}\\
%     &\geq \frac{v_i}{p_i} - H \frac{2\gamma + 3\alpha}{(1+\alpha)(1+\gamma)}\\
%     &\geq \frac{v_i}{p_i} - H \cdot \frac{2\gamma + 3\alpha}{2}.
% \end{align*}

% To get an error bound of $\epsilon$ it suffices to set $\gamma \leq \frac{\epsilon}{2H}$ and $\alpha \leq \frac{\epsilon}{3H}$ (which is a looser condition compared to the other direction). The sample complexity remains of $\tilde{O}\left(\frac{H^2}{\epsilon^2p_i}\right).$

% \textcolor{red}{END}

%\subsubsection{Estimating $[\E[v^*(\vec{x}) \mid \vec{x} \in \cS]$ from samples}

%Assume $v^\ast$ is known. We also know $\cS$. Given samples $\vx_1, \cdots \vx_m \in \cS$, we can calculate $v_1, \cdots, v_m$.

%Define the empirical CDF of $v^\ast(\vx) \mid \vx \in \cS$ with $m$ samples as 
%\[
%\hat F_m (v) = \frac{1}{m} |v_i: v_i \leq v|.
%\]
%Then, by the Dvoretzky-Kiefer-Wolfowitz (DKW) inequality, let $\epsilon = \sqrt{\frac{\log(2\delta^{-1})}{2m}}$, we have a guarantee that
%\[
%\Pr\left(\sup_{v \in [0,H]} |F(v) - \hat F(v)| \leq \epsilon \right) \geq 1-\delta.
%\]

%Moreover, for any $v\in [0,H]$,
%\[
%\widehat{F_m^{-1}}\left( \widehat{F_m}(v)\right) \leq v \leq \widehat{F_m^{-1}}\left( \widehat{F_m^{-1}}(v) + \frac{1}{m}\right).
%\]

%Using $\widehat{F_m^{-1}}$, we can sample from the distribution $\widehat{F_m}$ by inverse transform sampling:
%\begin{enumerate}
%    \item generate random sample $U \sim \text{Unif}[0,1]$
%    \item $V = \widehat{F_m^{-1}}(U)$
%\end{enumerate}

%Sample complexity of it?

% \subsubsection{Privacy preservation and lower bound on $p_i$}

% \paragraph{$K$-anonymous hashing.}

% Given $n$ samples $x_1, \cdots, x_n$, consider all subsets $\cS_i$ in which the input points have the same hash. We want to guarantee that 
% \[
% \argmin_i p_i = \E\left[\frac{\argmin_i|\cS_i|}{n}\right]\geq \beta.
% \] 
% This can be guaranteed using SortingLSH, which adds a post-processing procedure after the original SimHash.

% Define $K = \ceil{\beta n}$. SortingLSH generates cohorts as follows:

% \begin{itemize}
%     \item Sort $h_{\vec{w}}(\vec{x_1}), \cdots, h_{\vec{w}}(\vec{x_n})$ in lexicographical order.
%     \item Assign the sorted hashes to cohorts by partitioning the order
% in contiguous intervals containing at least $K$ users each.
% \end{itemize}

% This approach requires the sample size $n$ (or an upper bound of it) to be known to determine $K$.

% \paragraph{Deferentially private hashing.}

% This reference looks useful \url{https://arxiv.org/pdf/2010.09393.pdf}. \wg{still looking into it.}

==> sec/proof_finite.tex <==
\section{Proofs for Explore-then-Commit with Adversarial Prices} \label{app:finite-sample}

\estimateConditional*
\begin{proof}
Fix an index $i \in [n]$ such that $\eta_i \geq \beta$. We know that
\[\E\left[v^*(\vx) \mid h(\vx) = i\right] = \frac{\E[v^*(\vx) \Ind(h(\vx) = i)]}{\Pr[h(\vec{x}) = i]}.\] We use this fact to bound the difference between $\E\left[v^*(\vx) \mid h(\vx) = i\right]$ and $\frac{\hat{v}_i}{\hat{\eta}_i}$.

Beginning with the numerator, let $v_i = \E[v^*(\vx) \Ind(h(\vx) = i)]$, so $\hat{v}_i$ is an empirical estimate of $v_i$. Let $\alpha =  \sqrt{\frac{1}{\beta t'} \ln \frac{4n}{\delta}}$. By Bernstein's inequality~\citep[see, e.g.,][]{Haussler92:Decision}, with probability at least $1 - \frac{\delta}{2n}$, \begin{equation}\frac{(1 - \alpha)v_i - H\alpha\beta}{1 + \alpha} \leq \hat{v}_i \leq \frac{(1 + \alpha)v_i + H\alpha\beta}{1 - \alpha}.\label{eq:num}\end{equation}

Moving to the denominator, by a Chernoff-Hoeffding bound~\citep{boucheron2013concentration}, we know that with probability at least $1 - \frac{\delta}{2n}$, \begin{equation}\left(1 - 2\alpha\right)\eta_i \leq \hat{\eta}_i \leq \left(1 + 2\alpha\right)\eta_i.\label{eq:den}\end{equation} By definition of $\beta$, we know that $\alpha \leq \frac{1}{3}$, so $\hat{\eta}_i > 0$. 

We now bound the difference between $\E\left[v^*(\vx) \mid h(\vx) = i\right] = \frac{v_i}{\eta_i}$ and $\frac{\hat{v}_i}{\hat{\eta}_i}$, assuming that Equations~\eqref{eq:num} and \eqref{eq:den} hold, which we know that they do with probability at least $1- \frac{\delta}{n}$:
\begin{align*}\frac{\hat{v}_i}{\hat{\eta}_i} &\leq \frac{v_i}{\eta_i}\cdot \frac{1 + \alpha}{(1-\alpha)(1 - 2\alpha)} + \frac{H\alpha \beta}{\eta_i(1-\alpha)(1-2\alpha)}\\
&\leq \frac{v_i}{\eta_i}\cdot \frac{1 + \alpha}{(1-\alpha)(1 - 2\alpha)} + \frac{H\alpha }{(1-\alpha)(1-2\alpha)} &\left(\beta \leq \eta_i\right).\end{align*} Rearranging terms, we have that \begin{align}\frac{\hat{v}_i}{\hat{\eta}_i} &\leq \frac{v_i}{\eta_i}\cdot \left(1 + \frac{4\alpha - 2\alpha^2}{(1-\alpha)(1-2\alpha)}\right) + \frac{H\alpha}{(1-\alpha)(1-2\alpha)}\nonumber\\
&\leq \frac{v_i}{\eta_i}\cdot \left(1 + \frac{4\alpha}{(1-\alpha)(1-2\alpha)}\right) + \frac{H\alpha}{(1-\alpha)(1-2\alpha)}\nonumber\\
&\leq \frac{v_i}{\eta_i}\cdot \left(1 + 20\alpha\right) + 5H\alpha & \left(\alpha \leq \frac{1}{3}\right).\label{eq:rearrange}\end{align} Next, we use the fact that \[\frac{v_i}{\eta_i} = \frac{\E[v^*(\vx) \Ind(h(\vx) = i)]}{\Pr[h(\vec{x}) = i]} \leq \frac{\E[H \cdot \Ind(h(\vx) = i)]}{\Pr[h(\vec{x}) = i]} = \frac{H\Pr[h(\vec{x}) = i]}{\Pr[h(\vec{x}) = i]} = H.\] This inequality and Equation~\eqref{eq:rearrange} imply that \[\frac{\hat{v}_i}{\hat{\eta}_i} \leq \frac{v_i}{\eta_i} + 25H\alpha  = \frac{v_i}{\eta_i} + 25H\sqrt{\frac{1}{\beta t'}\ln \frac{4n}{\delta}}.\]

From the other direction, 
\begin{align*}
\frac{\hat{v}_i}{\hat{\eta}_i} &\geq \frac{v_i}{\eta_i} \cdot \frac{1-\alpha}{(1+\alpha)(1+2\alpha)}- \frac{H\alpha \beta}{\eta_i(1+\alpha)(1+2\alpha)}\\
&\geq \frac{v_i}{\eta_i} \cdot \frac{1-\alpha}{(1+\alpha)(1+2\alpha)}- \frac{H\alpha }{(1+\alpha)(1+2\alpha)} &(\beta \leq \eta_i).\end{align*}
Rearranging terms, we have that \begin{align*}
\frac{\hat{v}_i}{\hat{\eta}_i} &\geq \frac{v_i}{\eta_i} \left(  1 - \frac{4\alpha+2\alpha^2}{(1+\alpha)(1+2\alpha)}\right) - \frac{H \alpha }{(1+\alpha)(1+2\alpha)}\\
&\geq \frac{v_i}{\eta_i} - \frac{H(5\alpha+2\alpha^2)}{(1+\alpha)(1+2\alpha)} &\left(\frac{v_i}{\eta_i} \leq H\right)\\
&\geq \frac{v_i}{\eta_i} - \frac{7H\alpha}{(1+\alpha)(1+2\alpha)} &(\alpha < 1)\\
&\geq \frac{v_i}{\eta_i} - 7H\alpha &(\alpha \geq 0)\\
&= \frac{v_i}{\eta_i} - 7H\sqrt{\frac{1}{\beta t'}\ln \frac{4n}{\delta}}.\end{align*}

Therefore, the lemma statement holds by a union bound over all $i \in [n]$.
\end{proof}

\goodEvent*

\begin{proof}
For an arbitrary round $t \in \{t' + 1, \dots, T\}$ and an arbitrary pricing function $p_t : \cX \to [0,H]$, we will show that \[\E_{\vx_t \sim \cP}[ (v^\ast(\vx_t) - p_t(\vx_t))(s^*(h(\vx_t), p_t(\vx_t), h, \cP) - s_t(h(\vx_t), p_t(\vx_t)))] \leq H\left(25\sqrt{\frac{1}{\beta t'}\ln \frac{4n}{\delta}} + \beta n\right).\]
First, we decompose this expectation as \begin{align*}&\E_{\vx_t \sim \cP}[ (v^\ast(\vx_t) - p_t(\vx_t))(s^*(h(\vx_t), p_t(\vx_t), h, \cP) - s_t(h(\vx_t), p_t(\vx_t)))]\\
=& \E_{\vx_t \sim \cP}\left[ (v^\ast(\vx_t) - p_t(\vx_t))(s^*(h(\vx_t), p_t(\vx_t), h, \cP) - s_t(h(\vx_t), p_t(\vx_t))) \mid \eta_{h(\vx_t)} \geq \beta\right]\cdot \Pr_{\vx_t \sim \cP}\left[\eta_{h(\vx_t)} \geq \beta\right]\\
+& \E_{\vx_t \sim \cP}\left[ (v^\ast(\vx_t) - p_t(\vx_t))(s^*(h(\vx_t), p_t(\vx_t), h, \cP) - s_t(h(\vx_t), p_t(\vx_t))) \mid \eta_{h(\vx_t)} < \beta\right]\cdot \Pr_{\vx_t \sim \cP}\left[\eta_{h(\vx_t)} < \beta\right]\\
\leq &\E\left[ (v^\ast(\vx_t) - p_t(\vx_t))(s^*(h(\vx_t), p_t(\vx_t), h, \cP) - s_t(h(\vx_t), p_t(\vx_t))) \mid \eta_{h(\vx_t)} \geq \beta\right] + H\beta n.\end{align*}
The proof now follows by the same logic as the proof of Lemma~\ref{lem:loss-diff}, included below for completeness.

Now we bound the expected instantaneous regret in round $t$:
	\begin{align*}
	&\E_{\vx_t \sim \cP}\left[ (v^\ast(\vx_t) - p_t(\vx_t))(s^*(h(\vx_t), p_t(\vx_t), h, \cP) - s_t(h(\vx_t), p_t(\vx_t))) \mid \eta_{h(\vx_t)} \geq \beta\right]\\
	&= \E_{\vx_t \sim \cP}\left[\left. \E_{\vx \sim \cP}\left[(v^\ast(\vx) - p_t(\vx_t))(s^*(h(\vx_t), p_t(\vx_t), h, \cP) - s_t(h(\vx_t), p_t(\vx_t))) \mid h(\vx) = h(\vx_t)\right] \right| \eta_{h(\vx_t)} \geq \beta\right]\\
	&= \E_{\vx_t \sim \cP}\left[\left. \left(\E_{\vx \sim \cP}\left[v^\ast(\vx)\mid h(\vx) = h(\vx_t)\right] - p_t(\vx_t)\right)(s^*(h(\vx_t), p_t(\vx_t), h, \cP) - s_t(h(\vx_t), p_t(\vx_t))) \right| \eta_{h(\vx_t)} \geq \beta\right].\end{align*}
	
	Let $E$ denote the event where $s^*(h(\vx_t), p_t(\vx_t), h, \cP) \not= s_t(h(\vx_t), p_t(\vx_t))$. Then
	\begin{align*}
	&\E_{\vx_t \sim \cP}\left[ (v^\ast(\vx_t) - p_t(\vx_t))(s^*(h(\vx_t), p_t(\vx_t), h, \cP) - s_t(h(\vx_t), p_t(\vx_t))) \mid \eta_{h(\vx_t)} \geq \beta\right]\\
	&= \E_{\vx_t \sim \cP}\left[\left. \E_{\vx \sim \cP}\left[v^\ast(\vx)\mid h(\vx) = h(\vx_t)\right] - p_t(\vx_t) \right| E, \eta_{h(\vx_t)} \geq \beta\right] \cdot \prob_{\vx_t \sim \cP}[E]\\
	&\leq \E_{\vx_t \sim \cP}\left[\left. \left|\E_{\vx \sim \cP}\left[v^\ast(\vx)\mid h(\vx) = h(\vx_t)\right] - p_t(\vx_t)\right| \right| E, \eta_{h(\vx_t)} \geq \beta\right].
	\end{align*}
	
	Recall that \begin{align*}s^\ast(h(\vx_t), p(\vx_t), h, \cP) &= \Ind\left(\E_{\vx \sim \cP}\left[v^*(
\vx) \mid h(\vx) = h(\vx_t)\right] > p(\vx_t)\right)\\
s_t(h(\vx_t), p_t(\vx_t)) &= \Ind\left(\frac{\hat{v}_{h(\vx_t)}}{\hat{\eta}_{h(\vx_t)}} \geq p_t(\vx_t)\right).\end{align*}
	
Suppose that both the event $E$ happens and that $\eta_{h(\vx_t)} \geq \beta$. By the conditions of the lemma, the fact that $\eta_{h(\vx_t)} \geq \beta$ implies that $\hat{\eta}_{h(\vx_t)} > 0$. By definition of event $E$,
	\begin{align*}
		&\frac{\hat{v}_{h(\vx_t)}}{\hat{\eta}_{h(\vx_t)}}< p(\vec{x}) \leq \E_{\vx \sim \cP}[v^*(\vec{x}) \mid h(\vec{x}) = h(\vec{x}_t)], \text{ or}\\
		 	&E_{\vx \sim \cP}[v^*(\vec{x}) \mid h(\vec{x}) = h(\vec{x}_t)] < p(\vec{x}) \leq \frac{\hat{v}_{h(\vx_t)}}{\hat{\eta}_{h(\vx_t)}}.
	\end{align*}
	In either case we have that 
	\[
	\left|\E_{\vx \sim \cP}[v^*(\vec{x}) \mid h(\vec{x}) = h(\vec{x}_t)] - p(\vx) \right| \leq \left|\E_{\vx \sim \cP}[v^*(\vec{x}) \mid h(\vec{x}) = h(\vec{x}_t)] - \frac{\hat{v}_{h(\vx_t)}}{\hat{\eta}_{h(\vx_t)}} \right| \leq 25H\sqrt{\frac{1}{\beta t'}\ln \frac{4n}{\delta}},
	\]
		where the final inequality follows from the conditions of the lemma.
		
	Therefore, \[\E_{\vx_t \sim \cP}\left[\left. \left|\E_{\vx \sim \cP}\left[v^\ast(\vx)\mid h(\vx) = h(\vx_t)\right] - p_t(\vx_t)\right| \right| E, \eta_{h(\vx_t)} \geq \beta\right] \leq 25H\sqrt{\frac{1}{\beta t'}\ln \frac{4n}{\delta}},\] as claimed.
	\end{proof}

% \subsection{Proof for Lemma~\ref{lem:exp4-vc}}\label{app:proof-exp4-vcdim}

